Brownian Motions on Star Graphs with Non-Local Boundary Conditions

Brownian motions on star graphs in the sense of It\^o-McKean, that is, Walsh processes admitting a generalized boundary behavior including stickiness and jumps and having an angular distribution with finite support, are examined. Their generators are identified as Laplace operators on the graph subject to non-local Feller-Wentzell boundary conditions. A pathwise description is achieved for every admissible boundary condition: For finite jump measures, a construction of Kostrykin, Potthoff and Schrader in the continuous setting is expanded via a technique of successive killings and revivals; for infinite jump measures, the pathwise solution of It\^o-McKean for the half line is analyzed and extended to the star graph. These processes can then be used as main building blocks for Brownian motions on general metric graphs with non-local boundary conditions.

==> star_commands.tex <==
%% basic characters

\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}

\newcommand{\1}{\mathbbm{1}}	% indicator function

\newcommand{\PV}{\mathbb{P}}	% probability measure
\newcommand{\EV}{\mathbb{E}}	% expectation value

\newcommand{\cC}{\mathcal{C}}	% set of continuous functions

%\newcommand{\sC}{\mathscr{C}}	% sigma-algebra (general)
\newcommand{\sE}{\mathscr{E}}	% sigma-algebra (state space)
\newcommand{\sF}{\mathscr{F}}	% filtration (natural)
\newcommand{\sG}{\mathscr{G}}	% filtration (general)
\newcommand{\sS}{\mathscr{S}}	% set of excessive functions




% tilde~-characters
\newcommand{\tE}{\widetilde{E}}
\newcommand{\tsE}{\widetilde{\sE}}

% hat^-characters
\newcommand{\hO}{\hat{\Omega}}
\newcommand{\hE}{\hat{E}}
\newcommand{\hsE}{\hat{\sE}}
\newcommand{\hsF}{\hat{\sF}}
\newcommand{\hsG}{\hat{\sG}}
\newcommand{\hPV}{\hat{\PV}}
\newcommand{\hEV}{\hat{\EV}}
\newcommand{\hX}{\hat{X}}
\newcommand{\hT}{\hat{\Theta}}


%% math operators

\newcommand{\norm}[1]{\left\lVert #1 \right\rVert} % norm 

\newcommand\restr[2]{{		  	% restriction of a function
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 				  % the function
  \vphantom{\big|}		  % pretend it's a little taller at normal size
  \right|_{#2}    		  % this is the delimiter
  }}					
